Evaluation of a Region Proposal Architecture for Multi-task Document Layout Analysis

Automatically recognizing the layout of handwritten documents is an important step towards useful extraction of information from those documents. The most common application is to feed downstream applications such as automatic text recognition and keyword spotting; however, the recognition of the layout also helps to establish relationships between elements in the document which allows to enrich the information that can be extracted. Most of the modern document layout analysis systems are designed to address only one part of the document layout problem, namely: baseline detection or region segmentation. In contrast, we evaluate the effectiveness of the Mask-RCNN architecture to address the problem of baseline detection and region segmentation in an integrated manner. We present experimental results on two handwritten text datasets and one handwritten music dataset. The analyzed architecture yields promising results, outperforming state-of-the-art techniques in all three datasets.

==> Makefile <==
CAMERA = main

PAPER = main

SIZE      = letter
PLANT     = splncs04.bst llncs.cls
EXTS      = blg aux dvi log pdf ps bbl tex~ bib~ lot lof toc out maf mtc idx

POS=$(shell pwd)
PWD=$(notdir $(POS))

DIRFIG    := figs
EXTFIG    := jpg jpeg pdf_t pdf png eps ps
FIGSLST   := $(shell for I in $(EXTFIG); do find $(DIRFIG) -name "*.$$I"; done)

all:         pdf

.PHONY: pdf clean distclean
pdf:         $(PAPER).pdf

$(PAPER).aux: $(PAPER).tex $(PAPER).bib $(PLANT) $(FIGSLST)
	pdflatex $(PAPER)
	pdflatex $(PAPER)
	bibtex $(PAPER)
	pdflatex $(PAPER)
	pdflatex $(PAPER)

$(PAPER).pdf: $(PAPER).aux
	pdflatex $(PAPER)

clean:
	@rm -f $(foreach EXT,$(EXTS),*.$(EXT))

distclean: clean
	rm -vf $(PAPER).pdf


PDF: $(PAPER).pdf
	xpdf $<

PS: $(PAPER).ps
	gv $<

PACK: $(PAPER).tex $(PAPER).ps.gz $(PAPER).pdf $(PAPER).dvi $(PAPER).bib $(PLANT) Makefile $(FIGSLST)
#	cd ../; zip -r $(CAMERA) tex -x \*Makefile
#	cd ../; zip -r $(CAMERA) $(addprefix $(PWD)/, $^)
	cd ../; tar cvzhf $(CAMERA).tgz $(addprefix $(PWD)/, $^)

